A HRNet-based Rehabilitation Monitoring System

The rehabilitation treatment helps to heal minor sports and occupational injuries. In a traditional rehabilitation process, a therapist will assign certain actions to a patient to perform in between hospital visits, and it will rely on the patient to remember actions correctly and the schedule to perform them. Unfortunately, many patients forget to perform actions or fail to recall actions in detail. As a consequence, the rehabilitation treatment is hampered or, in the worst case, the patient may suffer from additional injury caused by performing incorrect actions. To resolve these issues, we propose a HRNet-based rehabilitation monitoring system, which can remind a patient when to perform the actions and display the actions for the patient to follow via the patient's smartphone. In addition, it helps the therapist to monitor the progress of the rehabilitation for the patient. Our system consists of an iOS app and several components at the server side. The app is in charge of displaying and collecting action videos. The server computes the similarity score between the therapist's actions and the patient's in the videos to keep track of the number of repetitions of each action. Theses stats will be shown to both of the patient and therapist. The extensive experiments show that the F1-Score of the similarity calculation is as high as 0.9 and the soft accuracy of the number of repetitions is higher than 90%.

==> 3_Preliminary.tex <==
\subsection{Human Pose Estimation}
\subsubsection{Open Source Computer Vision}
Open Source Computer Vision (OpenCV)~\cite{Culjak2012opencv} is the leading open-source library that has more than thousands of algorithms for computer vision, image processing, and machine learning. It is cross-platform and free for use in education, research, or commercial fields under the Apache 2 license. Furthermore, OpenCV runs on different operating systems such as Windows, Linux, Mac OS, iOS, and Android, and supports a wide variety of programming languages including C, C++, Java, and Python. The goal of OpenCV is to improve computational efficiency and provide a common infrastructure for developers. It makes the code more readable and transferable.

\subsubsection{High-Resolution Network}
In computer vision, human pose estimation is defined as the problem of localizing human joints.
High-Resolution Network (HRNet)~\cite{Sun2019HRNet} is a novel architecture which focuses on the following processes.
 \begin{enumerate}
   \item Maintaining reliable high-resolution representations through the whole process by connecting high-to-low resolution subnetworks in parallel.
   \item Repeatedly conducting multi-scale fusions across parallel convolutions for spatially precise heatmap estimation.
 \end{enumerate} 

Sun \etal~\cite{Sun2019HRNet} connect the multi-resolution subnetworks in parallel. They start with high-resolution subnetwork as the first stage and gradually add high-to-low resolution subnetwork in each stage. Thus, the resolution for the parallel subnetworks in the next stage is composed of the previous high resolution and lower one. The subnetwork \(\mathcal{N}_{sr}\) is in the \(s\)th stage and \(r\) is the resolution index. For instance, a possible network structure which contains 4 parallel subnetworks can be expressed as Equation~\ref{parallel_subnetworks}.
\begin{equation}
    \label{parallel_subnetworks}
    \begin{matrix} 
        \mathcal{N}_{11} & \longrightarrow & \mathcal{N}_{21} & \longrightarrow & \mathcal{N}_{31}\\
          & \searrow & \mathcal{N}_{22} & \longrightarrow & \mathcal{N}_{32}\\
          &   &   &  \searrow & \mathcal{N}_{33}
    \end{matrix}
\end{equation}

The network contains both high resolution subnetworks  (\(\mathcal{N}_{11} \longrightarrow \mathcal{N}_{21} \longrightarrow \mathcal{N}_{31}\)) and the compressed resolution subnetworks (\(\mathcal{N}_{11} \longrightarrow \mathcal{N}_{22} \longrightarrow \mathcal{N}_{33}\)).

The authors also introduce exchange unit, which aggregates the information from high to low resolutions of subnetwork in the current stage. There are two cases of fusion between different resolutions. For the high resolution, they adopt strided 3 × 3 convolutions to downsample for layer-by-layer. On the contrary, the upsampling of the simple nearest neighbor follows a 1 × 1 convolution to match the number of channels.

\subsection{Outlier Detection}
In statistics, the data points in a dataset that are extremely different from other data points are called outliers. They may cause serious problems and are difficult to explain in statistical analyses. Hence, outlier detection is an analysis for identifying and removing noisy data points from the dataset.

There are several causes for outliers, including sampling error, natural deviations, human error, or experimental error. For instance, measurement errors may cause incorrect values to be recorded from the experiment. Another example is that if the machine is out of order, it may produce random results. With extreme outliers, the data distribution may be skewed and has a disproportionate effect of the mean and standard deviation. 

Outlier detection takes into account the dimension of the feature. Outliers which occur within a single variable are univariate outliers. On the contrary, outliers which occur within multiple variables are multivariate outliers. Both of them have an ill effect on statistical analysis.

The most popular method for outlier detection is Z-Score. This method assumes that the variable has a Gaussian (normal) distribution. If a data point is above or below a given number of standard deviation from the mean, it indicates that the data point is an outlier. There are two situations to calculate a Z-Score, the formula for calculating the Z-Score is provided in Equation~\ref{z-score_p} in the case of population and Equation~\ref{z-score_s} in the case of samples:
    \begin{itemize}
      \item population:
            \begin{equation}
            \label{z-score_p}
                z = \frac{x-\mu}{\sigma},
            \end{equation}
        
            where \(x\) is the raw score, \(\mu\) is the mean of the population and \(\sigma\) is the standard deviation of the population.
    
      \item sample:
            \begin{equation}
            \label{z-score_s}
                z = \frac{x-\Bar{x}}{S},
            \end{equation}
            
            where \(x\) is the raw score, \(\Bar{x}\) is the mean of the sample and \(S\) is the standard deviation of the sample.
    \end{itemize}



\subsection{Noise Reduction}
Noise refers to different types of random or unwanted signals. There are many types of noises. In this paper, we focus on white noise, which is a random signal with equal intensity at diverse frequencies. White noise can also be used as a random number generator~\cite{Blum1986PseudoRandomNumberGenerator}. The process of removing noise from a target signal is called noise reduction. Noise reduction is important to recover a signal from an input waveform. In this section, we introduce two methods to reduce noise. 

\subsubsection{Savitzky–Golay filter}
A Savitzky–Golay filter (S–G filter)~\cite{savitzky64} is a digital filter which is widely used to smooth a set of digital data points and reduce noises. The main aim of S-G filter is to find a trend line for a given signal. Based on local linear least-squares polynomial approximation~\cite{LewisPolynomial}, a low-degree polynomial is used to fit consecutive subsets of adjacent data points.

\subsection{Kullback-Leibler Divergence}
In mathematical statistics and information theory, the Kullback-Leibler divergence (KL Divergence)~\cite{Kullback1968}, also known as relative entropy, represents a statistical distance that measures the divergence of a specific probability distribution from another referenced distribution. The definition of the KL divergence for discrete probability distributions \(P\) and \(Q\) within the same space \(\mathcal{X}\) is given in Equation~\ref{kl_discrete_1}.

If \(P\) and \(Q\) represent the probability distribution of a discrete random variable, the formula can be expressed as a summation:
    \begin{equation}
    \label{kl_discrete_1}
        D_{KL}(P \parallel Q) = \sum_{x\in\mathcal{X}}P(x)\log\left(\frac{P(x)}{Q(x)}\right)
    \end{equation}

%    non-negative是cite吉布斯不等式
An important property of KL divergence is that KL divergence is always non-negative, as shown in Equation~\ref{kl_non-negative}. Furthermore, when \(D_{KL}(P \parallel Q) = 0\), it means that \(P\) and \(Q\) are the same distribution.
    \begin{equation}
        \label{kl_non-negative}
           D_{KL}(P \parallel Q) \ge 0
    \end{equation}


% kl並不滿足距離的概念 因為1）不對稱2）不滿足三角不等式
However, KL divergence is not a true distance between two probability distributions since it is not symmetric. This means that the divergence of \(P\) from \(Q\) is not necessarily the same as \(Q\) from \(P\), which is shown in Equations~\ref{kl_asymmetric}.
    \begin{equation}
        \label{kl_asymmetric}
           D_{KL}(P \parallel Q) \neq D_{KL}(Q \parallel P)
    \end{equation}

